Providing Error Detection for Deep Learning Image Classifiers Using Self-Explainability

This paper proposes a self-explainable Deep Learning (SE-DL) system for an image classification problem that performs self-error detection. The self-error detection is key to improving the DL system's safe operation, especially in safety-critical applications such as automotive systems. A SE-DL system outputs both the class prediction and an explanation for that prediction, which provides insight into how the system makes its predictions for humans. Additionally, we leverage the explanation of the proposed SE-DL system to detect potential class prediction errors of the system. The proposed SE-DL system uses a set of concepts to generate the explanation. The concepts are human-understandable lower-level image features in each input image relevant to the higher-level class of that image. We present a concept selection methodology for scoring all concepts and selecting a subset of them based on their contribution to the error detection performance of the proposed SE-DL system. Finally, we present different error detection schemes using the proposed SE-DL system to compare them against an error detection scheme without any SE-DL system.

==> Tables/tab_dl_network_alex.tex <==
\setcounter{magicrownumbers}{0}

% \begin{smaller}


% \begin{table}
% \centering
% \smaller
% \caption{AlexNet Deep Learning Architecture}
% \label{tab:dl_net_arch_alex}
% \begin{tabular}[H]
% {>{\raggedright\arraybackslash}p{0.13\textwidth} >{\raggedright\arraybackslash}p{0.2\textwidth}>{\raggedright\arraybackslash}p{0.15\textwidth}>{\raggedright\arraybackslash}p{0.08\textwidth}>{\raggedright\arraybackslash}p{0.1\textwidth}>{\raggedright\arraybackslash}p{0.1\textwidth}}
% \hline
% \rowcolor[HTML]{93C47D} 
%  \textbf{Layer Type} & \textbf{Filter Size} & \textbf{HypParam.} & \textbf{\#Neurons} & \textbf{\#Weights} & \textbf{\#Operation} \\\hline\hline

% % ======================

% Conv.1  & number of filters=64, \newline filter size=$(11 , 11)$ & stride=4, \newline padding=2 &  200,704 &  23,232 &  72,855,552  \\ 
% Max Pooling & filter size=$(3 , 3)$ & stride=2, \newline padding=0&  &  &  \\ \hline

% Conv.2  & number of filters=192, \newline filter size=$(5 , 5)$ & stride=1, \newline padding=2  &139,968 & 307,200 & 223,948,800   \\ 
% Max Pooling & filter size=$(3 , 3)$ & stride=2, \newline padding=0&  &  &  \\ \hline

% Conv.3  & number of filters=384, \newline filter size=$(3 , 3)$ & stride=1, \newline padding=1  & 64,896 & 663,552 & 112,140,288   \\ \hline

% Conv.4  & number of filters=256, \newline filter size=$(3 , 3)$ & stride=1, \newline padding=1  & 43,264 & 884,736 & 149,520,384  \\ \hline

% Conv.5  & number of filters=256, \newline filter size=$(3 , 3)$ & stride=1, \newline padding=1  & 43,264 & 589,824 & 99,680,256  \\ 
% Max Pooling & filter size=$(3 , 3)$ & stride=2, \newline padding=0&  &  &  \\

% Avg. Pooling & filter size=$(6 , 6)$ &  & &  &  \\ \hline

% % Dropout & & $P_{dropout} = 0.5$ &  &  &  \\ \hline

% FC.1   & out features=4096  &  & 4,096 & 37,748,736 & 37,748,736\\ \hline

% FC.2   & out features=4096  &  & 4,096 & 16,777,216 & 16,777,216 \\ \hline
% Softmax & out features= $N+M$  & & 55 & 225,280 & 225,280 \\ \hline
% Total &  &  & 500,343 & 57,219,776 & 712,896,512 \\
% % ======================
% \hline
% \end{tabular}
% \end{table}
% \vspace{0.5cm}
% \end{smaller}
\begin{smaller}


\begin{table}
\centering
\smaller
\caption{Self-explainable and regular classifiers' architecture using AlexNet}
\label{tab:dl_net_arch_alex}
\begin{tabular}
% {c|c|c}
{>{\raggedright\arraybackslash}p{0.45\columnwidth} >{\raggedright\arraybackslash}p{0.27\columnwidth}>{\raggedright\arraybackslash}p{0.13\columnwidth}}
\hline
%\rowcolor[HTML]{93C47D} 
 \textbf{Layer Type} & \textbf{\#Filters, Filter Size} & \textbf{Hyper Parameter}  \\\hline\hline

% ======================

Convolutional Layer.1  & 64, (11 , 11) & stride=4,  padding=2 \\ \hline
Max Pooling & -, (3 , 3) & stride=2,  padding=0 \\ \hline

Convolutional Layer.2  & 192, (5 , 5) & stride=1,  padding=2  \\ \hline
Max Pooling & -, (3 , 3) & stride=2,  padding=0 \\ \hline

Convolutional Layer.3  & 384,(3 , 3) & stride=1,  padding=1  \\ \hline

Convolutional Layer.4  & 256, (3 , 3) & stride=1,  padding=1 \\ \hline

Convolutional Layer.5  & 256, (3 , 3) & stride=1,  padding=1 \\ \hline
Max Pooling & -, (3 , 3) & stride=2,  padding=0\\\hline

Avg. Pooling & -, (6 , 6) & \multicolumn{1}{c}{$-$}\\ \hline

% Dropout & & $P_{dropout} = 0.5$ &  &  &  \\ \hline

Fully Connected Layer.1   & out features=4096  & \multicolumn{1}{c}{$-$} \\ \hline

Fully Connected Layer.2   & out features=4096  & \multicolumn{1}{c}{$-$} \\ \hline
Softmax (Self-Explainable Classifier) & out features= $43+M^*$%, \newline $0\leq M^*\leq |\mathbb{A}^*|$
& \multicolumn{1}{c}{$-$}\\

Softmax (Regular Classifier) & out features= $43$ & \multicolumn{1}{c}{$-$}\\ \hline
% Total &  &  & 500,343 & 57,219,776 & 712,896,512 \\
% ======================
\hline
\end{tabular}
\end{table}
\vspace{0.5cm}
\end{smaller}


==> Tables/tab_dl_network_alex_comp.tex <==

\begin{smaller}
\begin{table}
\centering
\smaller
\caption{Computational Complexity Analysis of the regular and the proposed self-explainable classifiers.}
\label{tab:dl_net_arch_alex_comp}
\begin{tabular}
% {c|c|c|c}%[H]
{>{\raggedright\arraybackslash}p{0.43\columnwidth} >{\centering\arraybackslash}p{0.10\columnwidth}>{\centering\arraybackslash}p{0.12\columnwidth}>{\centering\arraybackslash}p{0.15\columnwidth}}
\hline
%\rowcolor[HTML]{93C47D} 
 \textbf{Layer Type} & \textbf{\#Neurons} & \textbf{\#Weights} & \textbf{\#Operation} \\\hline\hline

% ======================
Convolutional Layer.1    &   200,704   &   23,232   &   72,855,552  \\
Convolutional Layer.2    &   139,968   &   307,200   &   223,948,800  \\ 
Convolutional Layer.3    &   64,896   &   663,552   &   112,140,288  \\
Convolutional Layer.4    &   43,264   &   884,736   &   149,520,384  \\
Convolutional Layer.5    &   43,264   &   589,824   &   99,680,256  \\
Fully Connected Layer.1     &   4,096   &   37,748,736   &   37,748,736  \\
Fully Connected Layer.2     &   4,096   &   16,777,216   &   16,777,216  \\ \hline

Softmax (Self-Explainable Classifier)   &  
55   &   225,280   &   225,280  \\ 
Softmax (Regular Classifier)  &
43   &    176,128   &   176,128  \\ \hline

Total (Self-Explainable Classifier)   &
500,343   &   57,219,776   &   712,896,512  \\ 
Total (Regular Classifier)   &
500,331   &    57,170,624  &    712,847,360  \\
\hline\hline


% ======================

\end{tabular}
\end{table}
\vspace{0.5cm}
\end{smaller}

==> Tables/tab_dl_network_alex_time_analysis.tex <==

\begin{smaller}
\begin{table}
\centering
\smaller
\caption{Training and prediction times of the regular and the proposed self-explainable classifiers.}
\label{tab:dl_net_arch_alex_time_analysis}
\begin{tabular}
% {c|c|c}%[H]
{>{\raggedright\arraybackslash}p{0.25\columnwidth} >{\centering\arraybackslash}p{0.25\columnwidth}>{\centering\arraybackslash}p{0.25\columnwidth}}
\hline
%\rowcolor[HTML]{93C47D} 
 \textbf{Type of Classifier} & \textbf{Training time per iteration (sec.)} & \textbf{Prediction time per image (sec.)} \\\hline\hline

% ======================
% &&\\
Self-Explainable Classifier    &   8.669   &  0.002   \\ \hline
% &&\\
Regular Classifier   &   8.652   &   0.002   \\ 
% &&\\
\hline\hline


% ======================

\end{tabular}
\end{table}
\vspace{0.5cm}
\end{smaller}
